Compact Neural Representation Using Attentive Network Pruning

Deep neural networks have evolved to become power demanding and consequently difficult to apply to small-size mobile platforms. Network parameter reduction methods have been introduced to systematically deal with the computational and memory complexity of deep networks. We propose to examine the ability of attentive connection pruning to deal with redundancy reduction in neural networks as a contribution to the reduction of computational demand. In this work, we describe a Top-Down attention mechanism that is added to a Bottom-Up feedforward network to select important connections and subsequently prune redundant ones at all parametric layers. Our method not only introduces a novel hierarchical selection mechanism as the basis of pruning but also remains competitive with previous baseline methods in the experimental evaluation. We conduct experiments using different network architectures on popular benchmark datasets to show high compression ratio is achievable with negligible loss of accuracy.

==> 02-relatedwork.tex <==
Low-rank approximation, weight pruning, imposing sparsity through regularizers, and weight clustering are various approaches to reduce the number of learnable parameters in \convnets and other training-based systems.
%\textbf{Neural Network Compression:} 
\cite{denil2013predicting,denton2014exploiting} seek to find low-rank approximation of the weight kernel tensors by singular value decomposition. They achieve minimal performance degradation on large networks. These techniques are also computationally expensive and slow.
 \cite{han2016deep,chen2015compressing,park2017weighted} propose to cluster weights into a smaller number of groups that are representative of the original network. \cite{liu2015sparse,zhou2016less,wen2016learning} investigate the role of the sparsity-induced regularization terms such as L1-norm on the loss function. 

% \textbf{Weight Pruning:}
Weight pruning methods have been investigated from the early days of neural networks \cite{reed1993pruning}. \cite{lecun1990optimal,hassibi1993second} propose to prune the network connections based on the second-order derivatives of the loss function. The high computational complexity of computing the Hessian matrix on larger networks is a shortcoming of such methods. 
On the other hand, magnitude-based pruning \cite{han2015learning,guo2016dynamic,luo2017thinet} is fast, simple, and competitive with the baseline approaches. 
\cite{dong2017learning} recently proposes to compute the second derivatives of a reconstruction error minimization loss at each layer based on which the pruning is performed. 
All of these pruning methods uses retraining phase once a number of weights are set inactive for the subsequent steps. The number of pruning phases and the number of retraining iterations after a pruning phase to regain the same level of performance generalization are two important aspects of these methods.
We study the role of the selective attention introduced in STNet \cite{biparva2017stnet} for the task of weight pruning in neural networks. The selective attention mechanism defines stages of local competitions based on which a selection pattern over the network connections is generated at each layer. We propose the algorithm using which these patterns be harnessed for the determination of the weight pruning. The experimental evaluation reveals a competitive compression ratio and error rate after retraining with the baseline methods. 
